More Than Accuracy: Towards Trustworthy Machine Learning Interfaces for Object Recognition

This paper investigates the user experience of visualizations of a machine learning (ML) system that recognizes objects in images. This is important since even good systems can fail in unexpected ways as misclassifications on photo-sharing websites showed. In our study, we exposed users with a background in ML to three visualizations of three systems with different levels of accuracy. In interviews, we explored how the visualization helped users assess the accuracy of systems in use and how the visualization and the accuracy of the system affected trust and reliance. We found that participants do not only focus on accuracy when assessing ML systems. They also take the perceived plausibility and severity of misclassification into account and prefer seeing the probability of predictions. Semantically plausible errors are judged as less severe than errors that are implausible, which means that system accuracy could be communicated through the types of errors.

==> removed.tex <==
They wanted sufficient information to make an informed decision, which connects to a large body of research on the accountability of machine learning. Users take the plausibility and severity of misclassifications into account, which could motivate further research on how to expose ML systems to users in a way that focuses on their user experience. Future work could explore how to implement this in neural networks and other machine learning systems and how this affects the user experience.

 can only be the second step. First, an empirical basis for basic visualizations and their effect on the user experience of machine learning interfaces is needed.

 Our work is related to recent investigations of how to communicate algorithmic processes in online advertising, e.g. by explaining to users why an ad was shown to them~\cite{Eslami:2018:CAP:3173574.3174006}. 
